Smooth-AP: Smoothing the Path Towards Large-Scale Image Retrieval

Optimising a ranking-based metric, such as Average Precision (AP), is notoriously challenging due to the fact that it is non-differentiable, and hence cannot be optimised directly using gradient-descent methods. To this end, we introduce an objective that optimises instead a smoothed approximation of AP, coined Smooth-AP. Smooth-AP is a plug-and-play objective function that allows for end-to-end training of deep networks with a simple and elegant implementation. We also present an analysis for why directly optimising the ranking based metric of AP offers benefits over other deep metric learning losses. We apply Smooth-AP to standard retrieval benchmarks: Stanford Online products and VehicleID, and also evaluate on larger-scale datasets: INaturalist for fine-grained category retrieval, and VGGFace2 and IJB-C for face retrieval. In all cases, we improve the performance over the state-of-the-art, especially for larger-scale datasets, thus demonstrating the effectiveness and scalability of Smooth-AP to real-world scenarios.

==> arxiv_sec/B.tex <==
Following Section~4.1 in the main manuscript, here, we provide a quantitative analysis into the effect of sigmoid temperature $\tau$ on the tightness of the AP approximation.
%followed by an analysis into the exponential approximation and its links to some Deep Metric Learning methods. 
The tightness of the AP approximation can be computed by plotting the AP approximation error $AP_e$: 

\begin{align}
AP_e = |AP_{pred} - AP|,
\end{align}

\noindent where $AP_{pred}$ is the predicted approximate AP when the sigmoid is used in place of the indicator function in Equation 5~(from main manuscript), and $AP$ is the exact AP. 
We plot the AP approximation error over a training period for three different sigmoid temperatures~(Figures 2b, 2c, 2d in main manuscript), 
with the results shown in Figure~\ref{approx_fig}. 
As expected, a lower value of $\tau$ leads to a tighter approximation to Average Precision, 
as seen by the very low approximation error. 
This is as expected due to the convergence of the sigmoid towards the indicator function as $\tau$ decreases. 
As was shown in the ablation (Section 6.4 in main manuscript), 
there is a trade-off between a tight approximation to AP and a large enough operating region on the sigmoid such that a sufficient number of non-negligible gradients are fed back to the network.

\begin{figure}[!htb]
\begin{center}
   \includegraphics[width=0.55\linewidth]{eccv2020kit/supplementary_figures/approx.pdf}
\end{center}
\vspace{-10pt}
\beforecaptions
   \caption{\small{The AP approzimation error, $AP_e$ over one training epoch for different values of sigmoid annealing temperature, $\tau$. As can be seen, the lower the value of $\tau$ the tighter the approximation to AP. }}
 \aftercaptions
 \vspace{-1mm}
 \label{approx_fig}
\end{figure}


% $AP_pred$ is computed when the sigmoid when each of the differently annealed sigmoids is used in place of the indicator function in equation 5.


% By using each of the differently annealed sigmoid functions shown in figure 2 ($\tau$ = 0.1,0.01,0.001) in place of the indicator function in equation 5, we compute $AP_a$, 



% the approximate Average Precision (note that this is equivalent to equation x when the sigmoid approximation is used), and $AP_q$ (equation ... ) the true Average Precision when the discrete indicator function is used. We measure the approximation gap $AP_a - AP_q$ for each of the different approximations, over the model training period. Experiments are conducted on the CUB200 dataset, and in all cases the training conditions and parameters are kept constant, with only the indicator function approximation changing. As explained in section x, each iteration involves the computation of Average Precision when using each instance in the mini-batch in turn as a query, while the rest of the mini-batch acting as the retrieval set, so each measurement for Average Precision approximation is in fact the mean Average Precision approximation when averaged over each instance in the mini-batch.
\begin{comment}
\section{Exponential approximation to the indicator function}
%\section{Approximating AP with Neighborhood Component Analysis~(NCA)}
In order to be self-contained, 
we first review the definition of retrieval and how Average Precision~(AP) is computed mathematically.
Later, we show that the widely adopted Neighborhood Component Analysis~(NCA) can be treated as optimizing Recall@1 when the indicator function is replaced by an exponential function.
A formal proof is presented, showing that NCA only acts as an approximation of true AP, 
more precisely, it is optimizing for a lower bound of AP.

\subsubsection*{Task Definition.}
The goal of a retrieval system is to rank all instances in a retrieval set $\Omega = \{I_{i}, i = 0, \cdots, m\}$ based on their relevance to the query. 
For each query instance $I_q$, 
the retrieval set is split into the positive $\mathcal{P}_q$ and negative $\mathcal{N}_q$ sets, 
which are formed by all instances of the same class and of different classes, respectively. 
Note that there is a different positive and negative set for each query.

For a query $I_q$, 
the predicted relevance scores of all instances in the retrieval set are measured via a chosen metric. In our case, we use the cosine similarity (though the Smooth-AP method is independent of this choice):
\begin{align}
\mathcal{S}_{\Omega} = \left\{s_i = \left\langle \frac{v_q}{\|v_q\|} \cdot \frac{v_i}{\|v_i\|} \right\rangle, i = 0, \cdots, n\right\},
\end{align}
where $\mathcal{S}_{\Omega} = \mathcal{S}_P \cup \mathcal{S}_N$, 
and $\mathcal{S}_P = \{s_{\zeta}, \forall \zeta \in \mathcal{P}_q\}$, 
$\mathcal{S}_N = \{s_{\xi},   \forall \xi \in \mathcal{N}_q\}$
are the positive and negative relevance score sets, respectively, $v_{q}$ refers to the query vector, 
and $v_i, i = 0, \cdots, m $ to the vectorized retrieval set. 
The AP of a query $I_q$ is computed as:
\begin{align}  
\label{eq:AP_loss}
AP_{q} = \frac{1}{|\mathcal{S}_P|} \sum_{\substack{i \in \mathcal{S}_P}}
     \frac{\mathcal{R}(i, \mathcal{S}_P)}{\mathcal{R}(i, S_{\Omega})}, 
\end{align}
where $\mathcal{R}(i,\mathcal{S}_P)$ and $\mathcal{R}(i,\mathcal{S}_\Omega)$ refer to the rankings of the instance $i$ in $\mathcal{P}$ and $\Omega$, respectively. 
Note that, the rankings referred to in this paper are assumed to be \textit{proper rankings}, 
meaning no two samples are ranked equally.

\subsubsection*{Neighborhood Component Analysis~(NCA)~\cite{Goldberger05}} 
falls into the category of list-wise metric learning, 
with the goal of circumventing the combinatorial explosion in triplet sampling.
The idea is to contrast the positive pairs with multiple negative pairs,
and the objective can be summarized as:

\begin{align}
\mathcal{L} = \mathop{\mathbf{E}}_{I_q \in \Omega } \left[\tiny{-} \sum_{s_\zeta \in \mathcal{S}_P} \frac{\exp(s_\zeta)}{ \exp(s_\zeta) + \sum_{s_\xi \in \mathcal{S}_N}\exp(s_\xi)} \right]
\label{eq:listwise}
\end{align}

Intuitively, this allows a deep network to be trained for learnable k-nearst-neighbors, 
and has become popular in both the metric learning~\cite{Movshovitz17,Sohn16}
and the recent self-supervised learning community~\cite{Oord18,Henaff19,Hjelm19,Tian19, Ji19,He19,Han19,Zhuang19,Chen20}.
In this section, 
we prove that minimizing such an NCA loss is equivalent to optimizing a lower bound on the true AP.

For simplicity, we consider the single query $I_q$ case:
\begin{align}  
\label{eq:AP}
\mathcal{L}_{AP} 
& = \tiny{-} \sum_{\substack{s_\zeta\in\mathcal{S}_P}} 
    \frac{1+ \sum_{\epsilon \in \mathcal{S}_p ,\epsilon \neq \zeta} \mathbb{1}\{s_\epsilon - s_\zeta> 0\}}
       {1+ \sum_{\epsilon\in \mathcal{S}_P , \epsilon \neq \zeta} \mathbb{1}\{s_\epsilon - s_\zeta> 0\} 
       + \sum_{s_\xi \in \mathcal{S}_N } \mathbb{1}\{s_\xi - s_\zeta > 0\}} \nonumber \\
& = - \sum_{\substack{s_\zeta\in\mathcal{S}_P}} 
    \frac{1}
     {1 + \left(\sum_{s_\xi \in \mathcal{S}_N } \mathbb{1}\{s_\xi - s_\zeta > 0\} / (1+ \sum_{\epsilon\in \mathcal{S}_P , \epsilon \neq \zeta} \mathbb{1}\{s_\epsilon - s_\zeta> 0\}) \right)} 
\end{align}

\begin{align}
\mathcal{L}_{NCA} &= \tiny{-} \sum_{s_\zeta \in \mathcal{S}_P} \frac{\exp(s_\zeta)}{ \exp(s_\zeta) + \sum_{s_\xi \in \mathcal{S}_N}\exp(s_\xi)}  \nonumber \\ 
& = \tiny{-} \sum_{s_\zeta \in \mathcal{S}_P} \frac{1}{1 + \sum_{s_\xi \in \mathcal{S}_N}\exp(s_\xi - s_\zeta)} 
\label{eq:nca}
\end{align}
 
\noindent 
By observing Equation~\ref{eq:nca}, it is clear that $\mathcal{L}_{NCA}$ is indeed optimizing Recall@1,
with the indicator function being replaced with an exponential.
Meanwhile, consider the difference in the denominator between $\mathcal{L}_{NCA}$ and $\mathcal{L}_{AP}$,
\begin{align}
\delta &= exp(s_\xi - s_\zeta) - \frac{\mathbb{1}\{s_\xi - s_\zeta > 0\}} {1+ \sum_{\epsilon\in \mathcal{S}_P , \epsilon \neq \zeta} \mathbb{1}\{s_\epsilon - s_\zeta> 0\}} > 0 \nonumber \\
&\Longrightarrow \text{\hspace{10pt}} \mathcal{L}_{NCA} - \mathcal{L}_{AP} > 0~\text{(note the negative sign in the loss functions)} \nonumber
\end{align}

\noindent 
We can therefore draw the conclusion that the NCA loss acts as an upper bound for the AP loss, 
\ie~optimizing NCA loss is equivalent to optimizing a lower bound on the true Average Precision.

\end{comment}


==> table/faces_tab_fig.tex <==

% ===================== INIT TABLE ======================
\begin{table*}[ht]
\begin{minipage}[b]{0.6\textwidth}\centering
\small{
\begin{tabular}{l|cc}
\hline
Loss Function       & VF2 Test & IJB-C \\ \hline
VGGFace2            & 0.828    & 0.726 \\
VGGFace2 + Pair     & 0.828    & 0.728 \\
VGGFace2 + Triplet  & 0.845    & 0.740 \\
\textbf{VGGFace2 + Smooth-AP} & \textbf{0.850}     & \textbf{0.754} \\ \hline
ArcFace             & 0.858    & 0.772 \\
ArcFace + Pair      & 0.861    & 0.775 \\
ArcFace + Triplet   & 0.880    & 0.787 \\
\textbf{ArcFace + Smooth-AP}  & \textbf{0.902}    & \textbf{0.803} \\ \hline
\end{tabular}
}
\captionof{table}{\small{\textbf{mAP on face retrieval}. 
Smooth-AP {\em consistently} boosts the AP performance for both VGGFace2 and ArcFace, while outperforming the standard ranking losses (Pair and Triplet).}}
\label{tab:face_retrieval_results}
\end{minipage}
\hfill
\begin{minipage}[b]{0.39\textwidth}
    \centering
    \includegrap
    hics[width=0.89\textwidth]{eccv2020kit/figures/vic_faces3.pdf}
    \captionsetup{skip=0cm, width=0.95\textwidth}
    \captionof{figure}{\small{\textbf{Qualitative results on VGGFace2 testing set with Smooth-AP}. 
    For each query (top row), we display the top 3 instances, (all true positives).}}
    \label{fig:face_retrieval_results}
\end{minipage}
\end{table*}
